Search for scalar leptoquarks in $pp$ collisions at $\sqrt{s} = 13$ TeV with the ATLAS experiment

An inclusive search for a new-physics signature of lepton-jet resonances has been performed by the ATLAS experiment. Scalar leptoquarks, pair-produced in $pp$ collisions at $\sqrt{s}$ = 13 TeV at the Large Hadron Collider, have been considered. An integrated luminosity of 3.2 fb$^{-1}$, corresponding to the full 2015 dataset was used. First (second) generation leptoquarks were sought in events with two electrons (muons) and two or more jets. The observed event yield in each channel is consistent with Standard Model background expectations. The observed (expected) lower limits on the leptoquark mass at 95% confidence level are 1100 GeV and 1050 GeV (1160 GeV and 1040 GeV) for first and second generation leptoquarks, respectively, assuming a branching ratio into a charged lepton and a quark of 100%. Upper limits on the aforementioned branching ratio are also given as a function of leptoquark mass. Compared with the results of earlier ATLAS searches, the sensitivity is increased for leptoquark masses above 860 GeV, and the observed exclusion limits confirm and extend the published results.

==> SysTable.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{l|cc|c|c}
\midrule\midrule
\multirow{2}{*}{\bf Systematic uncertainties} & \multicolumn{2}{c|}{Signal Region}   & CR DY+jets &  CR $t\bar{t}$ \\ \cline{2-5}
     & Signal & Background  & Background &  Background \\
\noalign{\smallskip}\toprule\noalign{\smallskip}
%
Trigger S.F.                   & 10\%           & up to 1.5\%        & 3\%-4\%                  & 3\%-4\%                   \\
%
Electron Identification S.F.   & 8\%            & up to 2\%          & up to 1.5\%              & up to 1\%                 \\
%
Electron Isolation S.F.        & 2\%-7\%        & 2\%-3\%            & less than 1\%            & up to 2\%                 \\
%
JES$_{NP1}$                    & less than 1\%   & 3\%-4\%           & 6\%-8\%                  & 2\%-5\%                   \\
%
JES$_{NP2}$                    & less than 1\%   & up to 2\%         & 2\%-3\%                  & up to 2\%                 \\
%
JES$_{NP3}$                    & less than 1\%   & up to 2\%         & 2\%-3\%                  & up to 1.5\%               \\
%
\noalign{\smallskip}\midrule\midrule\noalign{\smallskip}
\end{tabular}
\end{center}
\caption[Breakdown of uncertainty in background estimates and expected signal]{
Breakdown of the dominant experimental systematic uncertainties in signal and background estimates in the signal region and for the background in the control regions, \ \eejj channel. The terms JES$_{NP1}$ , JES$_{NP2}$, and JES$_{NP3}$ refer to three nuisance parameters associated with the jet energy scale uncertainty. The abbreviation S.F. indicates scale factor. 
\label{table_syst_SR_ST600_eejj}}
\end{table}
%

\begin{table}[h!]
\begin{center}
\begin{tabular}{l|cc|c|c}
\midrule\midrule
\multirow{2}{*}{\bf Systematic uncertainties} & \multicolumn{2}{c|}{Signal Region}   & CR DY+jets &  CR $t\bar{t}$ \\ \cline{2-5}
     & Signal & Background  & Background &  Background \\
\noalign{\smallskip}\toprule\noalign{\smallskip}
%%
Trigger S.F.                   & up to 2\%      & up to 2\%          & 3\%-4\%                  & up to 1\%                 \\
%%
Muon Efficiency S.F.           & 4\%-8\%        & 2\%-4\%            & up to 1.5\%              & less than 1\%             \\
%%
Muon Isolation S.F.            & 2\%-7\%        & up to 1\%          & less than 1\%            & less than 1\%             \\
%%
JES$_{NP1}$                    & less than 1\%  & 2\%-5\%            & 6\%-7\%                  & 2\%-5\%                   \\
%%
JES$_{NP2}$                    & less than 1\%  & up to 2\%          & 2\%-3\%                  & 2\%-3\%                   \\
%%
JES$_{NP3}$                    & less than 1\%  & up to 2\%          & up to 4\%                & 1.5\%-2\%                 \\
%%
\noalign{\smallskip}\midrule\midrule\noalign{\smallskip}
\end{tabular}
\end{center}
\caption[Breakdown of uncertainty in background estimates and expected signal]{
Breakdown of the dominant experimental systematic uncertainties in signal and background estimates in the signal region and for the background in the control regions, \mumujj channel. The terms JES$_{NP1}$ , JES$_{NP2}$, and JES$_{NP3}$ refer to three nuisance parameters associated with the jet energy scale uncertainty. The abbreviation S.F. indicates scale factor.
\label{table_syst_SR_ST600_mumujj}}
\end{table}
%

